The $\gamma$-ray emitting region in low synchrotron peak blazars. Testing self-synchrotron Compton and external Compton scenarios

From the early days in gamma-ray astronomy, locating the origin of GeV emission within the core of an active galactic nucleus (AGN) persisted as an open question; the problem is to discern between near- and far-site scenarios with respect to the distance from the super massive central engine. We investigate this question under the light of a complete sample of low synchrotron peak (LSP) blazars which is fully characterized along many decades in the electromagnetic spectrum, from radio up to tens of GeV. We consider the high-energy emission from bright radio blazars and test for synchrotron self-Compton (SSC) and external Compton (EC) scenarios in the framework of localizing the $\gamma$-ray emission sites. Given that the inverse Compton (IC) process under the EC regime is driven by the abundance of external seed photons, these photons could be mainly ultraviolet (UV) to X-rays coming from the accretion disk region and the broad-line region (BLR), therefore close to the jet launch base; or infrared (IR) seed photons from the dust torus and molecular cloud spine-sheath, therefore far from jet launch base. We use enhanced SED information from recent works (including new $\gamma$-ray detections) to refine the study of Syn to IC peak correlations, which points to a particular $\gamma$-ray emission site. We show that SSC alone is not enough to account for the observed SEDs. Our analysis favors an EC scenario under the Thomson scattering regime, with a dominant IR external photon field. Therefore, the far-site (i.e., far from the jet launch) is probably the most reasonable scenario to account for the population properties of bright LSP blazars in cases modeled with a pure leptonic component. We calculate the photon energy density associated with the external field at the jet comoving frame to be $\rm U'_{ext}=1.69 \times 10^{-2}$ erg/cm$^3$, finding good agreement to other correlated works.

==> compton-longtable.tex <==
%LONG-TABLE-1
\begin{longtable}{llrcc|cccc}
%\centering
%\hspace*{-0.4cm}
\caption{Radio-Planck sample: Fitting parameters for the synchrotron and inverse Compton componentes. This is a measure of the mean SED, given all available data for each source}\\
\hline\hline
BZname          & R.A.        &  Dec.     &   Fluxrad2  & z   & Log($\nu$) & Log($\nu$f$_{\nu}$) & Log($\nu_{IC}$) &  Log($\nu$f$_{\nu-IC}$)  \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
BZname          & R.A.        &  Dec.     &   Fluxrad2  & z   & Log($\nu$) & Log($\nu$f$_{\nu}$) & Log($\nu_{IC}$) &  Log($\nu$f$_{\nu-IC}$)  \\
\hline
\endhead
\hline
\endfoot
 BZBJ0050-0929  &     12.67167 &    -9.48500 &    814.72058   &    0      &  14.6   &-11.0 & 22.7   &  -11.1       \\ 
 BZQJ1512-0905  &    228.21056 &    -9.09995 &   2701.6       &    0.360  &  13.1   &-10.9 & 22.2   &  -9.91       \\  
 BZQJ2229-0832  &    337.41705 &    -8.54847 &   968.85364    &    1.560  &  13.1   &-11.2 & 21.8   &  -10.5       \\  
 BZQJ0607-0834  &     91.99875 &    -8.58056 &   1905.8       &    0.870  &  12.1   &-11.5 & 21.4   &  -11.0       \\   
 BZUJ0241-0815  &     40.27000 &    -8.25576 &   913.254      &    0.005  &  13.5   &-10.1 & 20.9(?)&  -10.6       \\      
 BZQJ0808-0751  &    122.06473 &    -7.85275 &   1595.7       &    1.837  &  13.0   &-11.1 & 22.9   &  -10.7       \\       
 BZQJ0006-0623  &      1.55791 &    -6.39333 &   2051.4       &    0.347  &  13.0   &-11.1 & 20.3   &  -11.9       \\       
 BZQJ1256-0547  &    194.04652 &    -5.78931 &   9711.9       &    0.536  &  12.8   &-10.0 & 22.7   &  -10.0       \\      
 BZQJ2225-0457  &    336.44693 &    -4.95039 &   7411.7       &    1.404  &  13.0   &-10.8 & 21.7   &  -10.9       \\      
 BZQJ2218-0335  &    334.71683 &    -3.59358 &   2218.9       &    0.901  &  12.3   &-11.3 & 21.0   &  -11.7       \\      
 BZQJ1743-0350  &    265.99527 &    -3.83461 &   1411.4       &    1.057  &  12.6   &-11.3 & 21.0   &  -11.2       \\        
 BZBJ2134-0153  &    323.54294 &    -1.88812 &   1690.5       &    1.283  &  12.8   &-11.3 & 21.8   &  -11.5       \\        
 BZQJ0501-0159  &     75.30338 &    -1.98729 &   2264.9       &    2.291  &  13.0   &-11.4 & 21.4   &  -11.1       \\      
 BZQJ0339-0146  &     54.87891 &    -1.77667 &   2424.3       &    0.805  &  12.6   &-11.3 & 22.0   &  -11.1       \\         
 BZQJ0423-0120  &     65.81583 &    -1.34253 &   2726.5       &    0.916  &  13.0   &-10.6 & 22.1   &  -10.7       \\         
 BZUJ0725-0054  &    111.46125 &    -0.91556 &   1399.6       &    0.128  &  13.5   &-11.0 & 20.5   &  -11.2       \\         
 BZQJ0125-0005  &     21.37017 &    -0.09889 &   1540.8       &    1.077  &  12.8   &-11.6 & 20.3   &  -11.6       \\         
 BZQJ2136+0041  &    324.16080 &     0.69839 &   3473.1       &    1.941  &  11.7   &-11.6 & 21.2   &  -11.2       \\        
 BZQJ0108+0135  &     17.16154 &     1.58342 &   2621.3       &    2.099  &  12.9   &-11.2 & 22.4   &  -10.6       \\       
 BZQJ0739+0137  &    114.82513 &     1.61794 &   1964.9       &    0.189  &  13.9   &-10.9 & 21.6   &  -10.8       \\       
 BZUJ1058+0133  &    164.62338 &     1.56633 &   3220.8       &    0.890  &  13.1   &-10.9 & 22.3   &  -10.8       \\       
 BZQJ1229+0203  &    187.27792 &     2.05222 &   54992.       &    0.158  &  13.4   &-10.0 & 20.8   &  -9.54       \\         
 BZQJ1549+0237  &    237.37267 &     2.61700 &    836.24530   &    0.414  &  12.9   &-11.2 & 22.0   &  -11.1       \\           
 BZBJ0825+0309  &    126.45958 &     3.15667 &   1400.7       &    0.506  &  13.1   &-11.1 & 21.5(?)&  -11.6       \\           
 BZQJ1222+0413  &    185.59375 &     4.22083 &    800.87238   &    0.966  &  12.7   &-11.2 & 20.8   &  -10.7       \\           
 BZUJ0433+0521  &     68.29620 &     5.35433 &   3439.6       &    0.033  &  13.8   &-10.2 & 19.8   &  -10.2       \\         
 BZQJ2123+0535  &    320.93549 &     5.58947 &    794.14844   &    1.941  &  12.6   &-11.7 & 21.6   &  -11.8       \\            
 BZQJ1038+0512  &    159.69492 &     5.20808 &    640.43866   &    0.473  &  12.0   &-11.8 & 20.8   &  -12.1       \\          
 BZQJ1550+0527  &    237.64696 &     5.45290 &   2303.9       &    1.422  &  13.0   &-11.4 & 21.8   &  -11.4       \\
 BZQJ2148+0657  &    327.02252 &     6.96055 &   2590.0       &    0.999  &  12.5   &-10.8 & 20.5   &  -11.0       \\            
 BZUJ1751+0939  &    267.88675 &     9.65019 &    623.18988   &    0.322  &  13.1   &-10.8 & 21.9   &  -10.8       \\           
 BZBJ0757+0956  &    119.27766 &     9.94303 &    957.04303   &    0.266  &  13.7   &-10.8 & 20.8   &  -11.1       \\            
 BZQJ0309+1029  &     47.26500 &    10.48778 &    505.94873   &    0.863  &  12.8   &-11.2 & 21.7   &  -11.2       \\              
 BZQJ1608+1029  &    242.19249 &    10.48550 &   1392.6       &    1.226  &  12.8   &-11.3 & 21.6   &  -11.0       \\               
 BZQJ1504+1029  &    226.10408 &    10.49417 &   1774.8       &    1.839  &  12.8   &-11.6 & 22.9   &  -10.0       \\            
 BZQJ0010+1058  &      2.62917 &    10.97472 &     98.74014   &    0.089  &  14.5   &-10.7 & 20.5   &  -10.8       \\                
 BZBJ0449+1121  &     72.28196 &    11.35778 &    847.20898   &    2.153  &  12.9   &-11.5 & 21.8   &  -10.8       \\         
 BZQJ2232+1143  &    338.15167 &    11.73055 &   7202.1       &    1.037  &  12.4   &-11.2 & 21.3   &  -10.5       \\         
 BZQJ0750+1231  &    117.71687 &    12.51801 &   1487.0       &    0.889  &  12.6   &-11.1 & 21.2   &  -11.2       \\           
M87             &    187.70592 &    12.39111 &   1.38488E+05  &    0.0042 &  13.0   &-10.5 & 18.5(?)&  -10.4       \\              
 BZQJ0530+1331  &     82.73508 &    13.53200 &   1556.8       &    2.070  &  12.2   &-11.5 & 21.4   &  -10.7       \\         
 BZUJ1415+1320  &    213.99500 &    13.34000 &   1092.2       &    0.247  &  12.8   &-11.0 & 20.5   &  -11.2       \\         
 BZQJ2139+1423  &    324.75546 &    14.39333 &   1132.5       &    2.427  &  12.2   &-11.7 & -      &  -           \\            
 BZUJ0204+1514  &     31.21004 &    15.23639 &   4068.2       &    0.833  &  12.6   &-11.6 & 21.0   &  -11.2       \\           
 BZQJ2253+1608  &    343.49042 &    16.14805 &   12657.       &    0.859  &  13.1   &-10.0 & 22.2   &  -9.20       \\                
 BZBJ0238+1636  &     39.66167 &    16.61639 &   1941.9       &    0.940  &  13.0   &-10.9 & 22.5   &  -10.4       \\          
 BZQJ2203+1725  &    330.86203 &    17.43006 &    592.80420   &    1.076  &  13.3   &-10.9 & 22.9   &  -10.9       \\           
 BZBJ0738+1742  &    114.53083 &    17.70528 &   2258.3       &    0.424  &  13.5   &-10.6 & 23.8   &  -11.0       \\            
 BZQJ0510+1800  &     77.50988 &    18.01155 &    704.84467   &    0.416  &  13.3   &-11.3 & 21.3   &  -11.1       \\             
 BZBJ0854+2006  &    133.70332 &    20.10833 &   1512.4       &    0.306  &  13.6   &-10.4 & 21.8   &  -10.8       \\           
 BZQJ1224+2122  &    186.22713 &    21.37972 &   2095.2       &    0.434  &  13.1   &-10.7 & 23.0   &  -10.0       \\          
 BZQJ0152+2207  &     28.07525 &    22.11881 &   1041.7       &    1.320  &  12.9   &-11.5 & 21.8   &  -11.5       \\         
 BZQJ1327+2210  &    201.75359 &    22.18060 &    850.63739   &    1.398  &  12.6   &-11.7 & 21.7   &  -11.0       \\          
 BZQJ0830+2410  &    127.71700 &    24.18333 &    739.24634   &    0.939  &  12.6   &-11.1 & 21.8   &  -11.0       \\         
 BZQJ1043+2408  &    160.78749 &    24.14306 &    325.17075   &    0.560  &  12.9   &-11.5 & 21.7   &  -11.6       \\          
 BZQJ0956+2515  &    149.20784 &    25.25446 &   1080.7       &    0.712  &  12.7   &-11.4 & 21.9   &  -11.4       \\          
 BZQJ2236+2826  &    339.09363 &    28.48261 &   1103.4       &    0.790  &  13.0   &-11.2 & 22.5   &  -10.9       \\           
 BZQJ0237+2848  &     39.46838 &    28.80250 &   2197.5       &    1.206  &  12.9   &-11.2 & 22.0   &  -10.7       \\              
 BZQJ1159+2914  &    179.88263 &    29.24556 &   2031.7       &    0.729  &  13.5   &-11.1 & 22.6   &  -10.8       \\          
 BZQJ2203+3145  &    330.81210 &    31.76056 &   2879.4       &    0.295  &  13.4   &-10.9 & 20.9   &  -11.1       \\         
 BZQJ0336+3218  &     54.12542 &    32.30806 &   2677.2       &    1.259  &  12.8   &-11.3 & 20.2   &  -10.5       \\         
 BZUJ1310+3220  &    197.61940 &    32.34550 &   1687.2       &    0.997  &  13.1   &-10.8 & 22.2   &  -10.8       \\              
 BZQJ1613+3412  &    243.42084 &    34.21333 &   4024.7       &    1.397  &  12.3   &-11.5 & 21.7   &  -11.6       \\                  
 3C111          &     64.58867 &    38.02661 &   167.55414    &    0.0485 &  13.3   &-10.6 & 20.1   &  -10.0       \\         
 BZQJ1635+3808  &    248.81454 &    38.13458 &   2726.6       &    1.814  &  12.5   &-11.1 & 21.7   &  -10.3       \\               
 BZQJ1130+3815  &    172.72198 &    38.25514 &    702.57965   &    1.733  &  12.3   &-11.7 & 22.6   &  -11.6       \\           
 BZQJ0927+3902  &    141.76254 &    39.03914 &   2885.2       &    0.695  &  12.1   &-11.2 & -      &  -           \\           
 BZQJ0555+3948  &     88.87837 &    39.81366 &   1516.6       &    2.365  &  12.0   &-11.7 & 20.8   &  -10.9       \\           
 BZBJ1653+3945  &    253.46750 &    39.76000 &   1558.6       &    0.033  &  17.8   &-10.2 & 25.2   &  -10.6       \\            
 BZQJ1640+3946  &    250.12347 &    39.77898 &    977.31885   &    1.660  &  12.9   &-11.9 & 22.7   &  -10.8       \\          
 BZQJ1642+3948  &    250.74506 &    39.81028 &   7099.2       &    0.593  &  13.0   &-10.6 & 21.7   &  -10.7       \\         
 BZQJ2007+4029  &    301.93726 &    40.49683 &   2470.7       &    1.736  &  12.2   &-11.6 & -      &  -           \\             
 BZQJ0948+4039  &    147.23059 &    40.66239 &   1600.1       &    1.249  &  12.3   &-11.8 & 20.8   &  -11.2       \\             
 BZUJ0319+4130  & *   49.95042 &    41.51167 &   22830.0      &    0.018  &  13.0(?)&-10.4 & 23.3   &  -10.4       \\           
 BZBJ2202+4216  &    330.68042 &    42.27750 &   6051.5       &    0.069  &  13.6   &-10.0 & 21.3   &  -10.3       \\            
 BZUJ0909+4253  &    137.38959 &    42.89613 &   4234.4       &    0.670  &  12.9   &-11.5 & 20.9   &  -11.7       \\           
 BZQJ0646+4451  &    101.63346 &    44.85461 &    452.91037   &    3.396  &  11.6   &-11.8 & 21.8(?)&  -11.5       \\         
 BZQJ0920+4441  &    140.24359 &    44.69833 &   1017.8       &    2.190  &  12.5   &-11.2 & 22.3   &  -10.6       \\            
 BZQJ2354+4553  &    358.59033 &    45.88445 &   1872.8       &    1.992  &  12.2   &-11.9 & 21.4   &  -11.7       \\         
 BZQJ0136+4751  &     24.24412 &    47.85809 &   1138.1       &    0.859  &  13.3   &-10.9 & 22.2   &  -10.7       \\           
 BZUJ1829+4844  &    277.38251 &    48.74628 &   13753.       &    0.695  &  13.0   &-11.3 & 20.7   &  -11.1       \\            
 BZQJ1153+4931  &    178.35196 &    49.51911 &   1572.8       &    0.334  &  12.9   &-10.9 & 21.2   &  -11.1       \\                      
 BZQJ0808+4950  &    122.16529 &    49.84347 &   1115.1       &    1.432  &  12.0   &-12.2 & 20.6   &  -11.7       \\           
 BZQJ0359+5057  &     59.87396 &    50.96394 &   4296.7       &    1.512  &  12.1   &-10.7 & 21.3   &  -10.4       \\               
 BZQJ2038+5119  &    309.65433 &    51.32018 &   6081.3       &    1.686  &  12.5   &-11.5 & 21.4   &  -11.0       \\          
 BZQJ1955+5131  &    298.92810 &    51.53015 &   1588.2       &    1.214  &  12.7   &-11.7 & 20.7   &  -11.4       \\          
 BZQJ1740+5211  &    265.15408 &    52.19528 &    807.43494   &    1.381  &  13.2   &-11.3 & 21.3   &  -10.8       \\              
 BZBJ1419+5423  &    214.94417 &    54.38722 &    788.76880   &    0.153  &  13.7   &-10.6 & 21.9   &  -11.5       \\            
 BZBJ1824+5651  &    276.02948 &    56.85042 &   1412.3       &    0.663  &  13.2   &-11.3 & 22.1   &  -11.0       \\               
 BZUJ0102+5824  &     15.69067 &    58.40310 &    848.81873   &   ?0.644  &  12.6   &-11.1 & 21.8   &  -10.9       \\              
 BZQJ2022+6136  &    305.52783 &    61.61633 &   2093.7       &    0.228  &  12.9   &-11.2 & -      &  -           \\            
 BZBJ0958+6533  &    149.69666 &    65.56499 &    730.02911   &    0.367  &  13.4   &-11.0 & 21.2   &  -11.3       \\             
 BZQJ1849+6705  &    282.31833 &    67.09403 &    518.03430   &    0.657  &  13.1   &-10.9 & 22.5   &  -10.6       \\           
 BZQJ0228+6721  &     37.20854 &    67.35084 &   1540.6       &    0.523  &  12.8   &-11.2 & 21.1   &  -11.4       \\             
 BZQJ1642+6856  &    250.53271 &    68.94437 &   1720.8       &    0.751  &  12.5   &-11.6 & 20.1(?)&  -12.3       \\         
 BZBJ1806+6949  &    271.71124 &    69.82445 &   1887.2       &    0.046  &  14.0   &-10.6 & 21.7   &  -11.0       \\            
 BZQJ0841+7053  &    130.35153 &    70.89506 &   3823.8       &    2.218  &  12.4   &-11.3 & 20.1   &  -10.2       \\                  
 BZBJ0721+7120  &    110.47208 &    71.34333 &    727.30432   &    0.0    &  13.9   &-10.3 & 23.3   &  -10.5       \\         
 BZQJ0217+7349  &     34.37833 &    73.82555 &   2271.7       &    2.367  &  12.2   &-11.6 & 20.5   &  -10.4       \\           
% BZQJ1927+7358  &    291.95209 &    73.96711 &   3951.0       &    0.302  &  13.1   &-10.8 & 20.3   &  -11.0      \\
 BZQJ1927+7358  &    291.95209 &    73.96711 &   3951.0       &    0.302  &  13.1   &-10.8 & -      &  -           \\              
 BZBJ2005+7752  &    301.37961 &    77.87861 &   1060.8       &    0.342  &  13.2   &-11.2 & 21.5   &  -11.3       \\                
 BZBJ1800+7828  &    270.19034 &    78.46778 &   2223.6       &    0.680  &  13.5   &-10.7 & 21.9   &  -10.9       \\           
 BZQJ1153+8058  &    178.30208 &    80.97476 &   1343.5       &    1.250  &  12.6   &-12.0 & 21.1   &  -11.9       \\           
 BZQJ2356+8152  &    359.09497 &    81.88118 &    520.96356   &    1.344  &  12.8   &-11.8 & 21.1   &  -11.5       \\         


\label{tableRadioPlanck}
\end{longtable}

